A Quadratic Synchronization Rule for Distributed Deep Learning

In distributed deep learning with data parallelism, synchronizing gradients at each training step can cause a huge communication overhead, especially when many nodes work together to train large models. Local gradient methods, such as Local SGD, address this issue by allowing workers to compute locally for $H$ steps without synchronizing with others, hence reducing communication frequency. While $H$ has been viewed as a hyperparameter to trade optimization efficiency for communication cost, recent research indicates that setting a proper $H$ value can lead to generalization improvement. Yet, selecting a proper $H$ is elusive. This work proposes a theory-grounded method for determining $H$, named the Quadratic Synchronization Rule (QSR), which recommends dynamically setting $H$ in proportion to $\frac{1}{\eta^2}$ as the learning rate $\eta$ decays over time. Extensive ImageNet experiments on ResNet and ViT show that local gradient methods with QSR consistently improve the test accuracy over other synchronization strategies. Compared with the standard data parallel training, QSR enables Local AdamW on ViT-B to cut the training time on 16 or 64 GPUs down from 26.7 to 20.2 hours or from 8.6 to 5.5 hours and, at the same time, achieves $1.16\%$ or $0.84\%$ higher top-1 validation accuracy.

==> trash.tex <==
\section{Trash (Don't Read)}
%------------ unpolished -------------
\subsection{trash for theory}
We first compare the Slow SDEs for Local SGD with \mname and $H\sim\eta^{-1}$. Since $\widehat{\mSig}_{\Diamond}(\vzeta)$ is the upper limit of $\widehat{\mPsi}(\vzeta; H \eta)$ as $\beta=H\eta$ approaches infinity, \mname should drift faster towards flatter minima than $H\sim \eta^{-1}$. Keeping $H$ constant as $\eta$ diminishes to zero corresponds to setting the scaling factor $\beta$ in \eqref{eq:lsr-zeta} as a small value, making the extra drift term negligible and thus yielding nearly no generalization benefit over SGD. 
Based on Katzenberger's Theorem~\citep{kat}, \citet{li2021happens} showed that, if $\Phi(\vtheta_0) \in \Gamma$ for the initial point of SGD, then the gradient flow projections of SGD iterates $\Phi(\vtheta_t)$ over $O(\eta^{-2})$ steps converges in distribution to the following SDE, termed as Slow SDE, where each discrete step corresponds to a continuous time interval of length $\eta^2$ .
\citet{gu2023why} further provides quantitative analysis based on the method of moments, showing that this SDE provides an $\ctO(\eta^{0.25})$-weak approximation to SGD, namely that for any $\cC^3$-smooth function $g(\vtheta)$, the difference between the expected values of $g(\Phi(\vtheta_t))$ and $g(\vzeta(t\eta^2))$ is at most $\ctO(\eta^{0.25})$.



Based on the above interpretation of Slow SDE, \citet{gu2023why} conjectured that strengthening the drift term in the Slow SDE improves generalization.
One possible way is to increase the learning rate $\eta$ of SGD,
which makes one discrete step tracks longer continuous time,
hence increasing the drift term after a time rescaling.
However, using a very large $\eta$ can cause training instability and drive the parameter away from any minimizers. 
Alternatively, one can decrease the batch size $B$ since the drift term scales with $\frac{1}{2B}$.
However, each training step is more noisy as it consumes less data, and more steps and time are typically needed to reach the same training loss in the early phase.
Another issue is that the diffusion term in Slow SDE also increases, which can hinder the effect of the drift term.

%and a simple calculation can show that these operations do not change the relative scales of the drift and diffusion terms.
%less data parallelism can be used in distributed training, thus much longer wall-clock training time.

\myparagraph{Case II: Local SGD with $H \sim \eta^{-1}$.}
\citet{gu2023why} argued that performing Local SGD effectively strengthens the drift term of the Slow SDE while keeping the diffusion term unchanged. 
Consider the dynamics of Local SGD where $H = \beta / \eta$ for a constant $\beta$. That is, in each round of Local SGD, each worker locally diffuses around $\Gamma$ for $\sim \frac{1}{\eta}$ steps before averaging the parameter.
Since the local batch size is $K$ times smaller than the global one,
this local diffusion at each worker is much more significant than that in parallel SGD, and provably leads to an extra drift term in Slow SDE accumulated from higher-order terms in the local diffusion:


\citet{gu2023why} proved that the above SDE is an $\ctO(\eta^{0.25})$-weak approximation
of Local SGD. Here, the extra drift term scales with the matrix $\widehat{\mPsi}(\vzeta; \beta)$, which monotonically increases in $\beta$. When $\beta$ is small, $\widehat{\mPsi}(\vzeta; \beta) \approx \vzero$, so Local SGD is almost the same as parallel SGD for small $H$.
Conversely, if $\beta$ is very large,
$\widehat{\mPsi}(\vzeta; \beta) \approx \widehat{\mSig}_{\Diamond}(\vzeta)$. That is to say, the drift term of Local SGD with a large $\beta$ is approximately $K$ times that of parallel SGD, and hence, Local SGD can reduce sharpness faster than SGD.

Ideally, one should set $\beta$ to a maximal value to maximize the drift term. However, in practice, $\beta$ cannot be arbitrarily large. \citet{gu2023why} also showed that the distance between parameters and $\Gamma$ blows up as 
$\ctO(\sqrt{\beta \eta})$, suggesting that setting a very large $\beta$ for a not-so-small $\eta$ can blow up the loss.

%this approximation only holds rigorously for constant $\beta$. For large $\beta$, , 

\myparagraph{Case III: Local SGD with Quadratic Synchronization Rule.}
Instead of fixing $H$ or fixing $\beta = H \eta$, in QSR we dynamically adjust $H$ as $H = (\frac{\alpha}{\eta})^2$ for a small growth coefficient $\alpha$ (ignoring the floor function for simplicity).
This corresponds to blowing up $\beta$ as $\beta \sim \frac{1}{\eta}$ as $\eta \to 0$ in \citet{gu2023why}'s Slow SDE, so $\widehat{\mPsi}(\vzeta; \beta)$ converges to its upper limit, $\widehat{\mSig}_{\Diamond}(\vzeta)$, at small learning rate, which makes the total drift term $K$ times larger.
However, \citet{gu2023why}'s approximation theorem only holds in math for constant $\beta$.
In the following theorem, we rigorously establish the SDE approximation for Local SGD with QSR, confirming this view.
\kaifeng{our previous paper didn't prove this very rigorously, though it is simple.}
We defer the proof to \Cref{sec:proof-approx}.
%that the drift term is indeed $K$ times larger than that of parallel SGD.
%confirm with \citet{gu2023why}'s intuition that the drift term of Local SGD is $K$ times larger than parallel SGD.
%show that this indeed makes the drift term in the Slow SDE for Local SGD equal to $K$ times that for SGD.
% Amplifies the Drift Term.}


% \paragraph{A Toy Example.} $\cL(\theta_1, \theta_2)=0.5a\theta_1^2 (\theta_2^2 + b)$
\paragraph{Comparison of Different Scalings.} We first compare the Slow SDEs for Local SGD with \mname and $H\sim\eta^{-1}$. Since $\widehat{\mSig}_{\Diamond}(\vzeta)$ is the upper limit of $\widehat{\mPsi}(\vzeta; H \eta)$ as $\beta=H\eta$ approaches infinity, \mname should drift faster towards flatter minima than $H\sim \eta^{-1}$. Keeping $H$ constant as $\eta$ diminishes to zero corresponds to setting the scaling factor $\beta$ in \eqref{eq:lsr-zeta} as a small value, making the extra drift term negligible and thus yielding nearly no generalization benefit over SGD. In summary, the order of generalization performance predicted by our theory is: \mname $>$ $\{H\sim \eta^{-1}\}$ $>$ \{constant $H$\} $\approx$ parallel SGD. \longbo{do you want to make this a sentence by itself?}
% 
Notice that the last relationship may not apply to other optimizers such as AdamW, where the data parallel approach is not mathematically equivalent to setting $H=1$.
Experimental results in \Cref{fig:theory} validate that this generalization performance order of different scalings holds not only for SGD but also for AdamW. 
\subsection{Trash for intro}

Perhaps surprisingly, despite worse training loss, Local SGD has been observed to have 

increasing the number of local steps can sometimes lead to higher test accuracy.  \xinran{Say that larger H generalizes better than smaller H. Compare with local gradient methods with constant H instead of parallel SGD/ parallel AdamW} \cite{lin2020dont} discovered that compared with running standard SGD (equivalent to $H=1$) all through training, switching from SGD to Local SGD ($H>1$) at some time $t'$ consistently improves the final test accuracy. They term this approach \emph{Post-local SGD}. \xinran{rewrite}
%\cite{localadam} adopted Local Adam as a regularization technique and achieved higher test accuracy than Adam.
However, when this generalization benefit arises remains controversial. \cite{ortiz2021trade} reported that for multi-decay stepwise or cosine decay learning rate schedules, the regularization effect of Post-local SGD occurs only shortly after the switching point and diminishes in the end. Our observation aligns with theirs for Local SGD and Local AdamW in Figures 


Recently, from the generalization perspective, Lin et al...

This paper aims to improve the generalization of local gradient methods. A key message conveyed by Lin is that increasing $H$ can be used as a strong component to improve generalization with careful design. However, some questions remain unclear. (1) Post-local SGD always starts with $H=1$. Can we start with $H>1$ to reap the benefit of communication reduction? 
(2) Can we still observe the generalization benefit of increasing $H$ for adaptive gradient methods? (3) Ortiz et al.

Answer (1) - (3) one by one

While performing local updates significantly reduces the communication cost, it raises a concern that larger $H$ may lead to slower convergence of the training loss, posing a trade-off between optimization and communication efficiency \citep{khaled2020tighter, ortiz2021trade, lin2020dont} \xinran{Figure TBA}. 
%local gradient methods can sometimes beat standard gradient synchronization methods in test accuracy.


%\tba{Selecting H is an open problem, very difficult} Interestingly, despite worse training loss, increasing the number of local steps can sometimes lead to higher test accuracy.  \xinran{Say that larger H generalizes better than smaller H. Compare with local gradient methods with constant H instead of parallel SGD/ parallel AdamW} \cite{lin2020dont} discovered that compared with running standard SGD (equivalent to $H=1$) all through training, switching from SGD to Local SGD ($H>1$) at some time $t'$ consistently improves the final test accuracy. They term this approach \emph{Post-local SGD}. \xinran{rewrite}\cite{localadam} adopted Local Adam as a regularization technique and achieved higher test accuracy than Adam. However, when this generalization benefit arises remains controversial. \cite{ortiz2021trade} reported that for multi-decay stepwise or cosine decay learning rate schedules, the regularization effect of Post-local SGD occurs only shortly after the switching point and diminishes in the end. Our observation aligns with theirs for Local SGD and Local AdamW in Figures \xinran{TBA, multidecay schedule}. 
%\xinran{Using $H>1$ in the early phase is also our contribution. }
%the condition under which this generalization benefit arises remains a subject of debate
%provides new insights into

\xinran{briefly introduction the regularization effect here} Recently, \cite{gu2023why} sheds light on settling this debate by identifying the general condition for the generalization benefit of Local SGD to appear and developing a theoretical understanding of this benefit. They concluded via ablation studies that a smaller learning rate $\eta$ requires a higher number of local steps $H$ to maintain the regularization effect. This finding explains the transient improvement observed in \cite{ortiz2021trade}, where $H$ keeps unchanged after switching while $\eta$ decays multiple times. In Figures \xinran{TBA}, the generalization improvement indeed retains as we increase $H$ after $\eta$ decays. Furthermore, theoretical results in \cite{gu2023why} suggest that the optimal  $H$ for maximizing generalization should be at least $\Omega(\eta^{-1})$ (see Section \xinran{TBA} for a summary of their theory). 

%Inspired by
 Drawing upon the insights from \cite{gu2023why}, \kaifeng{swap this paragraph with the previous one; surprise people first, then tell them that we are actually inspired by a previous work} we propose a dynamic local step scheduling strategy aimed at improving the generalization of conventional local gradient methods that use a fixed number of local steps throughout training. We refer to local gradient methods with dynamic local step scheduling as``adaptive-step" and those without as``fixed-step" hereinafter. Our contributions are as follows:
 \xinran{easy, efficient, simple?}
 \xinran{should mention and explain 'regularization effect' earlier}
\begin{enumerate}
    \item We introduce a novel local step scheduling strategy that enhances the generalization performance of fixed-step local gradient methods. Our approach preserves the regularization effect  of local steps by enlarging $H$ in proportion to $\eta^{-1}$ \emph{raised to some power $\gamma$} as $\eta$ decays to a small value in the late phase of training. \kaifeng{merage it with the previous paragraph. That is, first surprise people that to improve the performance you need to increase the number of local steps rather than decrease it. Also cite some papers that suggest the opposite} As a byproduct of our approach, adaptive-step local gradient methods use much less communication in the late phase.
    \item We effectively address the training instability that occurs during transitions to larger values of $H$ by a novel and easy-to-implement ``learning rate quantization" strategy, which rounds the learning rate to powers of a predefined base. \xinran{Merge with the first point?}
    \item Theoretical results. subsume local versions of both SGD and adaptive gradient methods.
    \item We demonstrate through extensive empirical studies that our proposed local step scheduling consistently improves the generalization performance of fixed-step local gradient methods with various communication frequencies, even surpassing their standard gradient synchronization counterparts which induce much higher communication overhead.
    \item We validate the efficacy of our local step scheduling approach using a 64-GPU NVIDIA GeForce RTX 3090 cluster. As an illustrative example, standard AdamW takes 7.5 hours to train ViT-B for 300 epochs. In contrast, adaptive-step Local AdamW, enhanced with our dynamic local scheduling, cuts the training time down to \tba{TBA} hours with even higher test accuracy compared to standard AdamW.

    If the wall-clock time reduction is not that impressive, use this version: As an illustrative example, adaptive-step Local AdamW requires only \tba{TBA \%} of the communication frequency and achieves a high scaling efficiency of \tba{TBA}, with even higher test accuracy compared to standard AdamW. In contrast, the scaling efficiency of standard AdamW is only \tba{TBA}. 
    
    %We demonstrate the superiority of our local step scheduling on a 64-GPU NVIDIA GeForce RTX 3090 cluster. For example, while it takes 7.5 hours for standard AdamW to train ViT-B for 300 epochs, 
    % , adaptive-step Local AdamW equipped with our dynamic local scheduling reduces the training time 4.6 hours, achieving even higher test accuracy than standard AdamW. 
    % achieves \tba{TBA} scaling efficiency, 
    % with only \tba{TBA} of the communication volume
    % \xinran{Specify scaling efficiency, time reduction, communication volume reduction quantitatively}
\end{enumerate}
 
 
 We establish through comprehensive ablation studies that the optimal value of $\gamma$ for generalization falls within the range of $[1, 2]$. 
    %Additionally, we formulate a theoretical framework to corroborate our empirical observations regarding the optimal selection of \( \gamma \).

    We find via extensive ablation studies that the optimal power $\gamma$ for generalization lies in $[1,2]$.  We also develop a theory to justify our empirical finding about the optimal choice of $\gamma$.
  by inversely adjusting the number of steps $H_t$ according to the learning rate $\eta_t$ at the $t$-th step. Specifically, our approach starts with the base number of local steps $\constH$, and raises $H_t$ in proportion to powers of $\eta_t^{-1}$ as $\eta_t$ decays to a small value in the late phase of training.

 In our proposed scheduling, local step schedule inversely adjusts $H$ with the learning rate $\eta$. For fixed-step local gradient methods with the number of local steps $\constH$, we redefine the number of local steps at the $t$-th step based on the current learning rate $\eta_t$ as $H_t:=\max\left\{\constH, \left(\frac{\alpha}{\eta_t}\right)^{\gamma}\right\}$. Here, $\alpha $ and $\gamma$ are tunable constants. See \xinran{Algo TBA} for a formal description of our method. As shown in Figures \xinran{TBA}, employing this dynamic scheduling significantly enhances the generalization performance of fixed-step Local SGD and Local AdamW. 

adaptive-step local gradient methods

at the $t$-th step with learning rate $\eta_t$, we set the number of local steps $H_t=\max\left\{H_0,  \left(\frac{\alpha}{\eta_t}\right)^{\gamma}\right\}$, where $\alpha$ and $\gamma$ are constants to be tuned. This local step scheduling can improve the generalization performance of local gradient methods with constant $H_0$.
%"Fixed-Step Local Methods"
% "Constant-Step Local Gradient Methods"
% "Uniform-Step Local Methods"
% "Steady-Step Local Gradient Methods"

 %Our approach aims to optimize both communication efficiency and generalization performance in a coherent framework
%dynamically
%The reason behind the transient  is that $H$ is 
%indeed retains
%Furthermore, their theory indicates that the best  $H$ for generalization should be at least $\Omega(\eta^{-1})$ (see Section \xinran{TBA} for a summary of their theoretical results). 


%Via 


%The debate on the generalization benefit of local gradient methods has been recently reconciled by \cite{gu2023why}. 
%insighs from
%The success of local gradient methods in previous work indicates their potential to not only communicate little but also generalize well. 

% However, as suggested by \cite{ortiz2021trade}, reaping this generalization benefit is far from straightforward. 




%Our observations align with theirs when transitioning from a smaller to a larger $H$ in Local SGD and Local AdamW (see Figures \xinran{TBA}). 
%We observe a similar phenomenon as we switch from a smaller $H$ ($H>1$) to a larger one for Local SGD and Local AdamW 
%However, as \cite{ortiz2021trade} suggests, achieving this generalization benefit is nuanced. The regularization effect of Post-local SGD appears to be transient, manifesting shortly after the switch and ultimately fading away. Our findings align with this, observing a similar transient effect when adjusting the local step size $H$ in Local SGD and Local AdamW (see Figures \xinran{TBA}).
%reproduce their observation for Local SGD and Local AdamW with stepwise learning rate decay in Figures \xinran{TBA}.  
%Our observations align with this when transitioning from a smaller to a larger $H$ in Local SGD and Local AdamW (refer to Figures \xinran{TBA}).

%\cite{localadam} observed that Local Adam generalizes better than standard Adam.
%from cong et al: model averaging itself can also be an effective regularization measure

%While local gradient methods are usually known for their communication efficiency, they have also demonstrated the potential to improve the generalization performance of machine learning models. 
% While the primary advantage of local gradient methods has often been seen in their ability to reduce communication costs, their utility is not confined to this aspect alone. Interestingly, these methods have also demonstrated the potential to improve the generalization performance of machine learning models.

Gu et al studies vanilla SGD. This paper goes beyond SGD
key: maintain communication efficiency
\kaifeng{list experiments, must include the most highlighted experiments}


\begin{comment}
\subsection{Effectiveness of Learning Quantization}

key: LRQ $>$ No LRQ
Show train loss
\begin{enumerate}
    \item Directly applying our scheduling causes instability
    \item even add one step destabilize, 4 to 5
\end{enumerate}
\end{comment}




-------------------



Best improvement: ViT-B
Results for $B=4096$
\begin{enumerate}
    \item ViT-B, standard AdamW: 79.87; H=4: 79.26, H=4+adaptive steps: 80.9; H=8: 79.04, H=8+adaptive steps: 80.65.
    \item ResNet 152, SGDm: 79.57; H=4: 79.55, H=4+adaptive steps: 80; H=8: 79.35, H=8+adaptive steps: \tba{TBA}.
\end{enumerate}

Results for $B=16384$
\begin{enumerate}
    \item ViT-B, standard AdamW: 78.51; H=4: \tba{TBA}, H=4+adaptive steps: 79.46; H=8: \tba{TBA}, H=8+adaptive steps: \tba{TBA}
    \item ResNet 152, SGDm: 78.97; H=4: 78.14, H=4+adaptive steps: 78.81
\end{enumerate}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Method & Test Accuracy & Communication Frequency \\
        \hline
        SGD & 79.5 & 100\%\\
        Fixed-step Local SGD ($H=2$) & \tba{TBA} & \\
       \mname($\constH=2$) & \tba{TBA} &\\
Fixed-step Local SGD ($H=4$)& 79.5& 25\% \\
        \mname($\constH=4, \alpha=0.2$)  & 80& 20.5\%\\
        \hline
    \end{tabular}
    \caption{Results on ResNet-152.}
    \label{tab:resnet4k}
\end{table}
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Method & Test Accuracy & Communication Frequency \\
        \hline
        Standard AdamW & 79.5 & 100\% \\
        Fixed-step Local AdamW ($H=4$) & 79.26 &  25\% \\
        \mname ($\constH=4, \alpha=0.015$) & \textbf{80.9} & \textbf{12.7\%}\\
        Fixed-step Local AdamW ($H=8$) & 79.04 & 12.5\% \\
        \mname ($\constH=8, \alpha=0.015$) & \textbf{80.65} & \textbf{7.9\%}\\
        \hline
    \end{tabular}
    \caption{Results on ViT-B. The reported communication frequency for \mname is for the optimally tuned $\alpha$.}
    \label{tab:vit4k}
\end{table}




key:
\begin{itemize}
    \item dynamic $>$ const
    \item also compares with other baselines: standard gradient methods, either with batch size $B$ or $\constH B$
    \item if time is limited, run $\constH B$ only for 4096 $H=4$
\end{itemize}

\kaifeng{list experiments}


\subsection{Scaling Performance}\label{subsec:scaling efficiency}
\begin{table}
 \centering
    \begin{tabular}{@{} c |c |c| c @{}}
        \toprule
       Method & Comp (s). & Comm.(s) & Total (s)  \\
        \midrule
        Parallel SGD & 79.57\% & 1.57 & 100\%\\
        Local SGD ($H$=2) & 79.60\%& 1.58 &50\%\\
       Local SGD ($H$=4) &79.39\% &1.61 &25\%\\
       \midrule[0.2pt]
        QSR ($\constH=2$) & Entry 5 & Entry 6 &41.2\%\\
        QSR ($\constH=4$) & Entry 5 & Entry 6 &20.8\%\\
        \bottomrule
    \end{tabular}
    \captionof{table}{Per-iteration time breakdown and end-to-end runtime for ResNet-152 on 2x8 GPUs.}
\end{table}
\begin{minipage}{0.485\textwidth}
    \centering
    \begin{tabular}{@{} c |c |c| c @{}}
        \toprule
       Method & Test Acc. & Train loss & Comm.  \\
        \midrule
        Parallel SGD & 79.57\% & 1.57 & 100\%\\
        Local SGD ($H$=2) & 79.60\%& 1.58 &50\%\\
       Local SGD ($H$=4) &79.39\% &1.61 &25\%\\
       \midrule[0.2pt]
        QSR ($\constH=2$) & 80.34\% & Entry 6 &41.2\%\\
        QSR ($\constH=4$) & 80.3\% & Entry 6 &20.8\%\\
        \bottomrule
    \end{tabular}
    \captionof{table}{Per-iteration time breakdown and end-to-end runtime for ResNet-152 on 2x8 GPUs.}
\end{minipage}
\begin{minipage}{0.485\textwidth}
    \centering
    \begin{tabular}{@{} c| c |c |c @{}}
        \toprule
       Method & Test Acc. &  Train loss &  Comm.  \\
        \midrule
        Parallel AdamW & 79.65\% & 1.096 & 100\%\\
       Local AdamW ($H$=4) & 79.36\%& 1.03&25\%\\
       Local AdamW ($H$=8) &79.04\% & 1.07&12.5\%\\
       \midrule[0.2pt]
       QSR ($\constH=4$) & 81.03\% & Entry 6 &10.4\%\\
        QSR ($\constH=8$) & 80.66\% & Entry 6 &6.9\%\\
        \bottomrule
    \end{tabular}
    \captionof{table}{First table with bold lines.}
\end{minipage}

Batch size $16,384$. 

ResNet-152: communication:computation = 1:3
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        Method & Test Accuracy \\
        \hline
        SGD & 79.25\\
        Fixed-step Local SGD ($H=2$) & 78.85  \\
       \mname($\constH=2$) & 79.25 ($\alpha=0.2$) \\
Fixed-step Local SGD ($H=4$)& 78.34 \\
        \mname($\constH=4$)  & 78.68 ($\alpha=0.2$)\\
        \hline
    \end{tabular}
    \caption{Results on ResNet-152.}
    \label{tab:resnet16k}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        Method & Test Accuracy \\
        \hline
        Standard AdamW & 78.51 \\
        Fixed-step Local AdamW ($H=4$) & \tba{TBA}\\
        \mname ($\constH=4$) & 79.36 \\
        Fixed-step Local AdamW ($H=8$) & \tba{TBA} \\
        \mname ($\constH=8$) & 78.36 \\
        \hline
    \end{tabular}
    \caption{Results on ViT-B.}
    \label{tab:vit16k}
\end{table}

